Auto-Research Agent on MSA Organization to Improve Protein-Protein Complex Structure Prediction

Protein-complex structure prediction with AlphaFold 3 depends on MSA content, depth, and cross-chain pairing. Current pipelines apply uniform recipes, typically maximizing depth and pairing by species, yet even whether cross-chain pairing helps AF3 remains contested. We show that the value of both depth and pairing is strongly target-dependent, so no single recipe is optimal across interfaces. We introduce an autonomous agent that treats a frozen AF3 as a black-box experimental instrument. For each target, the agent formulates biological hypotheses, analyzes and reorganizes the MSA, and iteratively refines sequence selection and pairing using predictor label-free signals alone. On 1{,}015 protein--protein interfaces from three benchmarks released after AF3's training cutoff, the agent improves overall interface DockQ over AF3's default pipeline and fixed MSA recipes on every benchmark, while using on average 60\% fewer MSA sequences than the default. Gains are largest for inter-species heteromers, where species-based pairing is unreliable: mean DockQ increases from 0.465 to 0.612 on FoldBench and from 0.482 to 0.562 on HD439. The improvements arise from both sequence construction and pairing policy, including deliberate non-pairing. These results recast MSA design as a target-specific problem and show that an autonomous agent can adapt it at test time through biological reasoning and self-directed, confidence-guided experimentation.

==> sections/Methodology.tex <==
% ICLR-ready Methodology section derived from docs/method.md.
% Requires: \usepackage{amsmath,booktabs}

% \section{Methodology}
\label{sec:methodology}

Each episode contains exactly one protein-complex target.  The agent analyzes
the target-specific inputs, constructs candidate MSA pairings, evaluates them
through AlphaFold~3 (AF3), and ultimately selects one candidate that it
previously submitted successfully.  No memory is shared across targets and the
language model is not updated during an episode.

\subsection{Agent Execution Loop}
\label{sec:agent-loop}

We distinguish an \emph{experimental round} from an \emph{LLM turn}.  One
successful \texttt{submit} constitutes one round.  One invocation of the model
provider's \texttt{complete} interface constitutes one LLM turn, including
turns used for post-submit reflection or summary correction.  Internal route
failover within the provider does not create another agent-visible turn.

The runtime implements the following control flow.

\begin{enumerate}
\item \textbf{Active analysis.}
The model starts in the Active phase and may make zero or more ordinary tool
calls, primarily \texttt{analysis} and, when enabled, \texttt{uniprot}.  The
corresponding assistant messages and tool results remain in the live context
for the current round.

\item \textbf{Action requirement.}
The Active phase continues until the model calls \texttt{submit} or
\texttt{finish}.  A text-only reply has no effect on the environment.  In that
case, the runtime appends a new user-role message asking the model to continue
through a tool and requests another completion.

\item \textbf{Submission or termination.}
A valid \texttt{finish} must name a candidate from an earlier successful
submission.  It terminates the episode immediately, without another prediction
or reflection.  A \texttt{submit} must be the only tool call in its assistant
response.  If its arguments or candidate fail validation, the error is
returned as a tool result, the current context is retained, and execution
returns to Active.  Only a successful \texttt{submit} creates a new round and
consumes one evaluation.  The first successful submission must use
\texttt{layout: backend\_default} as the native control; manually row-aligned
candidates are permitted only afterward.

\item \textbf{Profile-visible feedback.}
After a successful \texttt{submit}, the host waits for AF3 inference, writes
the complete backend output to \texttt{/artifacts/<iteration>}, updates
\texttt{/observation/current.json}, and appends the feedback allowed by the
execution profile as the \texttt{submit} tool result.  In Blind episodes, this
feedback contains only AF3-native evidence; private ground-truth evaluation is
scheduled in the background and is not returned to the agent.  In GT-guided
episodes, \texttt{submit} also waits for the evaluator and returns its result.

\item \textbf{Reflection steer.}
Once the \texttt{submit} result is in the conversation, the runtime appends a
new user-role prompt requesting a summary of the completed round and invokes
the model again.  This operation steers the same conversation into
post-submit Reflection.  It does not modify the system prompt or start a new
episode.

\item \textbf{Post-submit reflection.}
During Reflection, the tool list contains only \texttt{analysis}.  The model
may call it zero or more times and may inspect any mounted evidence from the
current or an earlier round.  It cannot call \texttt{submit} or
\texttt{finish} until reflection is complete.

\item \textbf{Memory validation.}
The first reflection response without a tool call is parsed as a round-memory
JSON object.  If the object is invalid, the runtime appends a new user-role
correction prompt, preserves the complete reflection context, and invokes the
model again.  This loop continues until the JSON is valid or the global
LLM-turn budget is exhausted.

\item \textbf{Memory commit and context reset.}
The validated entry is appended to the episode's cumulative memory.  The live
context is then replaced by the original system message and one user-role
message containing every round-memory entry accumulated so far.  Messages from
the completed round are no longer sent to the model, although the offline
transcript and sandbox files remain intact.

\item \textbf{Return to Active.}
The model may conduct more analysis, submit another candidate, or call
\texttt{finish}.  The \texttt{next\_step} text stored in memory is advisory: it
does not drive a runtime transition and does not automatically invoke
\texttt{finish}.
\end{enumerate}

The principal path is therefore
\begin{equation}
\begin{aligned}
\mathrm{Active}
&\xrightarrow{\texttt{submit}}
\mathrm{Feedback},\\
\mathrm{Feedback}
&\xrightarrow{\mathrm{user\ steer}}
\mathrm{Reflection},\\
\mathrm{Reflection}
&\xrightarrow{\mathrm{valid\ memory}}
\mathrm{Context\ reset}
\longrightarrow \mathrm{Active}.
\end{aligned}
\label{eq:agent-loop}
\end{equation}
A successful \texttt{finish} is a separate terminal edge directly from Active
and bypasses submission, inference, and reflection.

Every model-provider completion counts toward the LLM budget, and every
successful \texttt{submit} counts toward the evaluation budget.  Tool calls are
recorded, but the runtime imposes no separate tool-call budget.  If the model
exhausts its completion budget without a valid \texttt{finish}, the episode
fails rather than silently selecting a candidate.

\subsection{Analysis Sandbox and Persistent Files}
\label{sec:sandbox}

The \texttt{analysis} tool accepts a purpose and a complete Python program.  The
host first saves the source under
\texttt{<case\_output\_dir>/workspace/analysis}, using
\texttt{<analysis\_id>.py} as its name, and then runs it in an isolated process.
Inside that process, the same file is visible as
\texttt{/workspace/analysis/<analysis\_id>.py}.  The latter is the sandbox path
observed by the agent; the host's absolute path is not exposed.

Table~\ref{tab:sandbox-paths} lists the principal mounts.  ``Episode''
persistence means that the contents survive analysis calls, experimental
rounds, and context resets for the current target, but are not shared with
another target.

\begin{table*}[t]
\centering
\caption{Paths available to agent-written analysis code.}
\label{tab:sandbox-paths}
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabular}{p{0.23\textwidth}p{0.11\textwidth}p{0.48\textwidth}p{0.11\textwidth}}
\toprule
\textbf{Path} & \textbf{Access} & \textbf{Contents} & \textbf{Lifetime} \\
\midrule
\texttt{/input} & Read-only & Public case, chain, sequence, and MSA data for the
current target. & \raggedright Episode \tabularnewline
\texttt{/observation/}\newline\texttt{current.json} & Read-only & Remaining evaluation budget,
successful-submission history, and profile-visible feedback. &
\raggedright Per successful submission \tabularnewline
\texttt{/artifacts/}\newline\texttt{<iteration>} & Read-only & Complete native outputs from each
successful AF3 inference. & \raggedright Episode; append-only \tabularnewline
\texttt{/artifacts/}\newline\texttt{research} & Read-only & Research records released by the
optional host coordinator; analysis code cannot create files here. &
\raggedright Episode; append-only \tabularnewline
\texttt{/workspace} & Read--write & Agent-authored programs, candidates, notes,
tables, and figures. & \raggedright Episode \tabularnewline
\texttt{/tmp} & Read--write & Scratch space local to one \texttt{analysis}
process. & \raggedright One analysis call \tabularnewline
\texttt{/ground\_truth} & Read-only & Private reference and evaluation data. &
\raggedright GT-guided only \tabularnewline
\bottomrule
\end{tabular}
\end{table*}

The phrase ``inspect the current round's artifacts'' does not restrict
reflection to that round.  An \texttt{analysis} call may read the public input,
the current observation, every AF3 artifact directory from iteration 001
through the current iteration, and all programs, candidates, and notes retained
in \texttt{/workspace}.  GT-guided episodes additionally mount
\texttt{/ground\_truth}.  Unmounted host directories remain inaccessible.  In
particular, host-side evaluator outputs under \texttt{/evaluations} are never
mounted, preventing a Blind agent from opening hidden DockQ results.

Each \texttt{analysis} call runs in a fresh Python process for at most 120
seconds.  Socket creation and direct network access are blocked; external
information must be obtained through an explicitly registered coordinator
tool.  The process may write persistent results to \texttt{/workspace}, whereas
\texttt{/tmp} is local to the current call.

For the AF3 backend, each artifact directory contains the exact
\texttt{input.json} used for that submission, the backend \texttt{run.log}, the
top-ranked structure and confidence files, and the per-seed/per-sample CIF,
full-confidence, PAE, and summary-confidence files.  The agent may use these
outputs to study cross-sample stability, chain-pair ipTM, PAE, pLDDT, contacts,
predicted geometry, and clashes.

\subsection{System Prompt and Dynamic Context}
\label{sec:system-prompt}

The system prompt is compiled once at episode initialization from three blocks
in a fixed order,
\begin{equation}
P = P_{\mathrm{task}}
\oplus P_{\mathrm{backend}}
\oplus P_{\mathrm{sandbox}}.
\label{eq:system-prompt}
\end{equation}
The task block specifies the target-specific MSA-pairing objective, suggested
analysis directions, experimental loop, and candidate constraints.  The
backend block explains how the local AF3 backend consumes candidates, the
semantics of its MSA channels, the generated artifacts, model-native feedback,
and the Blind/GT feedback boundary.  The sandbox block defines visible paths,
permissions, and lifetimes.  Their concatenation is the complete system prompt
and remains unchanged for the entire episode.

Four other components are deliberately kept outside the system prompt.  Tool
schemas are passed through the model API on each LLM turn; target data reside
under \texttt{/input}; history and remaining budget reside in
\texttt{/observation/current.json}; and accumulated memory is supplied after a
reset as one user-role \texttt{episode\_memory} message.  Consequently, under a
fixed backend, Blind and GT-guided runs use the same system prompt.  Their
difference is realized by the actual mounts and feedback filter.

\subsection{Registered Tools and Candidate Validation}
\label{sec:tools}

Table~\ref{tab:tools} summarizes the registered tools and their phase
availability.

\begin{table*}[t]
\centering
\caption{Registered agent tools.  Only a successful \texttt{submit} consumes
an evaluation.}
\label{tab:tools}
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabular}{p{0.12\textwidth}p{0.13\textwidth}p{0.13\textwidth}p{0.12\textwidth}p{0.37\textwidth}}
\toprule
\textbf{Tool} & \textbf{Active} & \textbf{Reflection} &
\textbf{Evaluation cost} & \textbf{Function} \\
\midrule
\texttt{analysis} & Available & Available & None & Executes a complete Python
program and returns its saved path, exit code, standard output, standard error,
and timeout status. \\
\texttt{uniprot} & Optional & Unavailable & None & Requests screened background
information about non-target homologs through a bounded host coordinator. \\
\texttt{submit} & Available & Unavailable & One on success & Reads and validates
a candidate in \texttt{/workspace}, runs AF3, and returns profile-visible
feedback. \\
\texttt{finish} & Available & Unavailable & None & Records a final choice and
conclusion for a previously successful candidate; runs no new inference. \\
\bottomrule
\end{tabular}
\end{table*}

A failed \texttt{analysis} still returns its diagnostics to the live context,
allowing the model to repair the program.  The optional \texttt{uniprot} tool
is a screened retrieval interface rather than unrestricted Internet access; it
makes approved records available under \texttt{/artifacts/research} and is not
exposed during Reflection.

The \texttt{submit} arguments are a candidate path inside \texttt{/workspace}
and a non-empty experimental summary.  For a
\texttt{manual\_row\_aligned} candidate, the host checks the public chain keys,
exact query sequences, A3M row lengths after lowercase insertion characters are
removed, and equal record counts across chains before invoking AF3.  Record
$i$ across the per-chain A3Ms denotes the intended paired row $i$.  Validation
failures do not consume the evaluation budget or create a round.

The \texttt{finish} arguments are a previously submitted
\texttt{candidate\_id} and a non-empty conclusion.  The tool records that
selection and terminates the episode; it does not infer a new structure.
Argument or protocol errors from any tool are returned as structured error
results and remain in the current context for subsequent correction.

\subsection{Post-submit Reflection Memory}
\label{sec:memory}

Every successful \texttt{submit} must be followed by exactly one memory entry.
The reflection prompt tells the model that the named candidate has completed,
identifies the round number, permits optional inspection of backend artifacts
through \texttt{analysis}, and prohibits another \texttt{submit} or
\texttt{finish} before reflection completes.  It then requests only one JSON
object with the fields shown in Table~\ref{tab:memory-schema}.  The prompt also
instructs the model not to copy raw Python, tool output, or large metric tables
into memory.

\begin{table*}[t]
\centering
\caption{Canonical round-memory schema.  The runtime adds \texttt{round}; the
model supplies the remaining fields.}
\label{tab:memory-schema}
\small
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabular}{p{0.24\textwidth}p{0.50\textwidth}p{0.17\textwidth}}
\toprule
\textbf{Field} & \textbf{Content} & \textbf{Validation} \\
\midrule
\texttt{round} & \raggedright Index of the completed successful submission. &
\raggedright Runtime-added \tabularnewline
\texttt{candidate\_id} & \raggedright Identifier of the candidate just completed. &
\raggedright Exact match \tabularnewline
\texttt{approach} & \raggedright Concise description of the tested construction
and hypothesis. & \raggedright Non-empty \tabularnewline
\texttt{observations} & \raggedright Direct observations from profile-visible
feedback and mounted artifacts. & \raggedright 1--5 items \tabularnewline
\texttt{scientific\_}\newline\texttt{findings} & \raggedright Current scientific
conclusions, including negative results. & \raggedright 1--4 items \tabularnewline
\texttt{engineering\_}\newline\texttt{lessons} & \raggedright Reusable
implementation or processing lessons. & \raggedright 0--3 items \tabularnewline
\texttt{uncertainties} & \raggedright Counterevidence and unresolved questions. &
\raggedright 0--4 items \tabularnewline
\texttt{next\_step} & \raggedright Proposed next experiment or reason to finish. &
\raggedright Non-empty \tabularnewline
\bottomrule
\end{tabular}
\end{table*}

The runtime validates the exact field set, verifies that
\texttt{candidate\_id} matches the completed submission, checks list and field
lengths, adds \texttt{round}, and serializes the canonical object as compact
JSON.  Each entry is limited to 4,000 Unicode characters.  If validation fails,
the runtime appends a correction prompt reporting the error and asks the model
to return a corrected JSON object.  This is another steer in the same
Reflection context: preceding feedback and analysis results are retained.

After validation, the entry $M_t$ is appended to an ordered, append-only memory
list.  The runtime resets the live model context to exactly
\begin{equation}
\begin{aligned}
J_t &= \{\texttt{episode\_memory}:[M_1,\ldots,M_t]\},\\
C_{t+1} &= [P,\;U(\operatorname{serialize}(J_t))],
\end{aligned}
\label{eq:memory-reset}
\end{equation}
where $P$ is the original system message and $U(\cdot)$ denotes one user-role
message.  Memory is not inserted into or used to rewrite the system prompt.
The 4,000-character limit applies to each $M_t$, not to the cumulative array;
the memory message therefore grows with the number of successful submissions.

The \texttt{next\_step} field is natural-language working memory for the next
Active phase, not a runtime command.  For example, a value such as ``Finish and
select candidate X'' does not terminate the episode.  After reset, the model
may revise that plan, continue analyzing, or submit another experiment.  Only
an actual successful \texttt{finish} tool call is terminal.

Context reset changes what is sent to the model, not what is stored.  Earlier
Python programs remain in \texttt{/workspace/analysis}; candidates and notes
remain in \texttt{/workspace}; AF3 outputs remain in
\texttt{/artifacts/<iteration>}; and removed assistant/tool messages remain in
the offline \texttt{conversation.json}.  Persisted files must be reopened
explicitly with \texttt{analysis} if the model needs their detailed contents in
a later round.

\subsection{Blind Feedback and Final Evaluation}
\label{sec:blind-evaluation}

In the Blind condition, every value in \texttt{submit.feedback.model} and every
file under the AF3 artifact directory is derived from the candidate input or
AF3's predictions.  The compact feedback contains the mean and maximum AF3
\texttt{ranking\_score}, ipTM, and pTM across generated samples, while the full
prediction tree remains available for analysis.  AF3
\texttt{ranking\_score} is a backend-native confidence quantity: it is neither
computed by the agent nor obtained by comparing a prediction with ground
truth.

Blind feedback contains no DockQ, iRMSD, lRMSD, success label, evaluator report,
or other ground-truth-derived quantity.  AF3 confidence, PAE, pLDDT, contacts,
and predicted geometry may inform comparisons among candidates, but they are
predictions rather than measurements of native structural accuracy.  Because
ground-truth feedback is unavailable, the Blind agent must decide what to test
and which candidate to select from public input, AF3-native evidence, persistent
workspace records, and its own analysis.

The host nevertheless evaluates every successful submission privately with
the configured FoldBench/OpenStructure evaluator.  Let $z_t$ be the AF3 output,
$m_t$ its model-native feedback, and $e_t$ the private evaluator report.  The
profile-visible feedback is
\begin{equation}
f_t^{(p)} =
\begin{cases}
m_t, & p=\mathrm{blind},\\
(m_t,e_t), & p=\mathrm{GT\text{-}guided}.
\end{cases}
\label{eq:profile-feedback}
\end{equation}
In Blind runs, $e_t$ is computed asynchronously after AF3 and may overlap
post-submit reflection or the next GPU inference.  In GT-guided runs,
\texttt{submit} waits for $e_t$ because it is visible and may causally affect
the next action.

For the AF3--FoldBench2 protein-interface task, the primary score is
\begin{equation}
\mathrm{score}(c_t)=\mathrm{dockq\_mean}(c_t).
\label{eq:primary-score}
\end{equation}
DockQ is first averaged over the evaluated seed/sample predictions for each
configured interface and then averaged across the evaluated interfaces in the
case.  At the end of a Blind episode, the host waits for all outstanding
evaluator tasks, but reports the score only for the candidate selected by the
agent's \texttt{finish} call.  Hidden DockQ values are never used to re-rank the
trajectory or substitute an oracle candidate for the agent's choice.

\subsection{Trajectory Records}
\label{sec:trajectory-records}

The implementation retains both the host-side experimental record and the
subset of information that was visible to the agent.  The principal outputs
are:
\begin{itemize}
\item \texttt{conversation.json}: the complete system, user, assistant, and
tool transcript, including messages later removed from the live context;
\item \texttt{checkpoint.json}: the current phase, live messages, full
transcript, accumulated memories, call counts, and other recovery state;
\item \texttt{result.json}: the final candidate and conclusion, all completed
iterations, their round memories, and host-side offline evaluations; and
\item \texttt{artifacts/<iteration>/run.log}: the AF3 backend log for each
successful submission.
\end{itemize}
Because \texttt{conversation.json} includes messages from contexts that were
subsequently reset, it is an audit transcript rather than a representation of
any one model request.  The current logs record cumulative LLM- and tool-call
counts, but do not record a start time, end time, or elapsed duration for each
individual LLM turn.

